SCStory: Self-supervised and Continual Online Story Discovery

We present a framework SCStory for online story discovery, that helps people digest rapidly published news article streams in real-time without human annotations. To organize news article streams into stories, existing approaches directly encode the articles and cluster them based on representation similarity. However, these methods yield noisy and inaccurate story discovery results because the generic article embeddings do not effectively reflect the story-indicative semantics in an article and cannot adapt to the rapidly evolving news article streams. SCStory employs self-supervised and continual learning with a novel idea of story-indicative adaptive modeling of news article streams. With a lightweight hierarchical embedding module that first learns sentence representations and then article representations, SCStory identifies story-relevant information of news articles and uses them to discover stories. The embedding module is continuously updated to adapt to evolving news streams with a contrastive learning objective, backed up by two unique techniques, confidence-aware memory replay and prioritized-augmentation, employed for label absence and data scarcity problems. Thorough experiments on real and the latest news data sets demonstrate that SCStory outperforms existing state-of-the-art algorithms for unsupervised online story discovery.

==> 7.Limitations.tex <==
\section{Limitations}
While \algname{} demonstrated its effectiveness in a typical unsupervised online story discovery task, we discuss some limitations worth exploring for future work as follows.

First, the definition of a story can be more relaxed. While an article usually belongs to a single story in real cases, there might be some cases where an article could belong to multiple stories. For instance, an article is under a unique story but may cover the related stories together in a balanced way. An article may also comprehensively overview different stories in the same timeline. The stories discovered by \algname{} may need to be post-processed for merging or splitting to refine those cases. Alternatively, a fundamental extension of \algname{} towards soft clustering (i.e., multiple cluster memberships) or hierarchical clustering with a correspondingly customized model update policy (e.g., multi-label contrastive learning) is worth exploring.

Second, the temporal scope for story discovery can be dynamically considered. Typical real stories consist of articles published consistently for a long time (i.e., long-term stories) or only for a few days (i.e., short-term stories), which can be discovered through the sliding window. However, if there are sparse stories with articles very rarely published for a long period of time (e.g., an incident of which investigation process proceeds very slowly), the sparse stories will be easily expired from a sliding window so that the continuity of the stories will not be preserved. In this case, we may need to design a supplementary offline repository for managing such sparse stories, in conjunction with the sliding window. Note that simply considering the wider temporal scope (e.g., a landmark window or a memory replay from all previous articles), which we also discussed in the experiment, may not be an effective solution as this will harm the efficiency as well as the recency of the model to deal with unbounded article streams.

Third, while \algname{} effectively exploits the generalized embedding capability of a PSE, it is also dependent on the PSE which provides a base embedding space for self-supervision. To complement this, a weak-supervision with a very few true story labels or story-relevant information (e.g., a topic or category name included in the metadata of an article) could be effective but efficient guidance for \algname{} to boost its performance as well as to mitigate the dependency on the base PSE.

%Besides the aforementioned points, we also believe that considering the applicability of \algname{} in various domains of target article streams other than the news domain or exploring the compatibility of \algname{} with different types of PLMs could be interesting topics for future work.

==> Figures/Ablation_others.tex <==
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
  & \multicolumn{4}{c}{News14} & \multicolumn{4}{c}{WCEP18} & \multicolumn{4}{c}{WCEP19} \\
  & $B^{3}$-P   & $B^{3}$-R    & AMI & ARI   & $B^{3}$-P   & $B^{3}$-R    & AMI & ARI & $B^{3}$-P   & $B^{3}$-R    & AMI & ARI   \\ \midrule
\rowcolor{lightgray}
\algname{} (default)   
& \textbf{0.887}
& \textbf{0.871}
& 0.879 & \textbf{0.809} &0.828 &\textbf{0.851} &\textbf{0.884} &0.757 & 0.848&0.843 &\textbf{0.892} &\textbf{0.781} \\
\ w/o memory replay (MR)  & 0.883             & 0.861    &    0.875  & 0.798&  \textbf{0.839} & 0.808 &0.874 &0.752 & \textbf{0.858} & 0.801 & 0.881 & 0.769\\
\ w/o prioritized-aug. (PA)    &  0.883           & 0.857       &  0.873  & 0.799 &0.824 &0.846 &0.881 &0.753 &0.815  &\textbf{0.853} &0.883 &0.745    \\
\ w/o MR \& PA  &0.884 &0.851 &0.873 &0.799               &  0.827      &  0.807  &0.869 &0.742 &0.840 &0.805 &0.877 &0.760   \\
\ w/o story-indicative emb.  &    0.871          &   0.842   & 0.868  & 0.797 & 0.793 & 0.75& 0.834&0.686 &0.805  & 0.750&0.846 &0.711    \\\midrule
\algname{} with MR from  &              &        &      & & & & & & & & & \\
\ last two windows   &    0.885          &  0.866      &0.877     & 0.803&0.819 &0.849 &0.880 &0.748 &0.839 &0.845 &0.889 &0.769\\
\ last three windows & 0.884  &0.866              & 0.877       &0.803    &0.822 &0.850 &0.883 &0.754 &0.835 &0.845  &0.888 & 0.765 \\
\ all previous windows & 0.886             & \textbf{0.871}      &\textbf{0.881}      & 0.808&0.829 &0.850 & \textbf{0.884}& \textbf{0.760}& 0.853 & 0.839 & \textbf{0.892}  & 0.779\\ \midrule
\algname{} with PA by   &             &        &     & & & & & & & & & \\
\ Attentive pooling weights  &  0.885           &   0.861 &  0.875  & 0.800 & 0.822 &0.846 &0.881 &0.753 &0.839 &0.831 &0.886 &0.766\\
\ Random sentence shuffle  & 0.884           & 0.866     &0.877  & 0.805&0.818 &0.851 &0.880 &0.749 &0.842 &0.838 &0.889 &0.771 \\
\ Random feature dropout   &  0.882      &0.868     & 0.877   &0.803 &0.812 &0.852 &0.878 &0.744 &0.826&0.850 &0.887 &0.760\\ \midrule
{\renewcommand{\arraystretch}{0.8} \begin{tabular}[l]{@{\!}l@{\!}}\!\algname{} updated only\\ \!once with the first window\end{tabular}} &   0.856           &  0.869       &  0.869   & 0.789 &0.753 &0.809 &0.844 &0.685 & 0.776& 0.810&0.857 &0.719 \\
\bottomrule
\end{tabular}


==> Figures/ChanttanoogShooting.tex <==
\fbox{\begin{minipage}{\textwidth}
{\footnotesize
\begin{itemize}[label={},leftmargin=0pt, noitemsep]
\item \underline{ 2022-06-05 }
\item \textbf{Title}: Police: Tennessee shooting leads to 3 dead, 14 injured
\item 	\textbf{Top sentence (weight: 0.143)}: A shooting near a Tennessee nightclub early Sunday led to three deaths and 14 people suffering gunshot wounds and other injuries, police said.
\vspace{0.05cm}
\item \underline{ 2022-06-06 }
\item \textbf{Title}: Police: Tennessee shooting leads to 3 dead, 14 injured
\item 	\textbf{Top sentence (weight: 0.18)}: CHATTANOOGA, Tenn. — A shooting near a Tennessee nightclub early Sunday led to three deaths and 14 people suffering gunshot wounds and other injuries, police said.
\vspace{0.05cm}
\item \underline{ 2022-06-09 }
\item \textbf{Title}: Man arrested on weapons charge in Tennessee mass shooting
\item 	\textbf{Top sentence (weight: 0.171)}: CHATTANOOGA, Tenn. — One man has been arrested on a weapons charge in a mass shooting over the weekend in Chattanooga, Tennessee, where three people died and 14 were injured.
\vspace{0.05cm}
\item \underline{ 2022-06-11 }
\item \textbf{Title}: Police identify 3 killed in Tennessee mass shooting
\item 	\textbf{Top sentence (weight: 0.126)}: Police identify 3 killed in Tennessee mass shooting
\vspace{0.05cm}
\end{itemize}
}
\end{minipage}}

==> Figures/Covid19Pandemic.tex <==
\fbox{\begin{minipage}{\textwidth}
{\footnotesize
\begin{itemize}[label={},leftmargin=0pt, noitemsep]
\item \underline{ 2022-06-01 }
\item \textbf{Title}: `Covid-Pop’ Is a New Genre, and Loudon Wainwright III Brings the Latest Addition
\item \textbf{Top sentence (weight: 0.124)}: If nothing else, the virus has found common ground between genres that otherwise would have barely much in common.
\vspace{0.05cm}
\item \underline{ 2022-06-02 }
\item \textbf{Title}: COVID deaths in Africa to fall by 94\% in 2022: WHO
\item \textbf{Top sentence (weight: 0.234)}: Although African countries struggled early in the pandemic to secure COVID-19 vaccines as rich countries hoarded available doses, many are now well-supplied with shots but are having trouble getting them into arms.
\vspace{0.05cm}
\item \underline{ 2022-06-03 }
\item \textbf{Title}: : Starbucks stores in Shanghai welcome customers as COVID lockdown eases
\item \textbf{Top sentence (weight: 0.121)}: In the most recent fiscal second-quarter earnings, Starbucks reported a 23\% decline in comparable sales in China, with comparable transactions down 20\%.
\vspace{0.05cm}
\item \underline{ 2022-06-04 }
\item \textbf{Title}: COVID-19 Ontario: Hospitalizations at 671, ICU admissions near 100 | CTV News - CTV News Toronto
\item \textbf{Top sentence\!(weight: 0.113)}:In the ICU, 60 patients are fully vaccinated, 10 are unvaccinated, and four are partially vaccinated.\!
\vspace{0.05cm}
\item \underline{ 2022-06-05 }
\item \textbf{Title}: ATO says COVID tests could be a deduction
\item \textbf{Top sentence (weight: 0.153)}: With the end of the financial year looming, the ATO expects COVID-19 will continue to impact tax returns.
\vspace{0.05cm}
\item \underline{ 2022-06-06 }
\item \textbf{Title}: Coronavirus pandemic led to £140bn-worth of ‘forced saving’
\item \textbf{Top sentence (weight: 0.049)}: This compares with a household saving ratio of just 6.0\% between October and December 2019, before any lockdown restrictions were imposed.
\vspace{0.05cm}
\item \underline{ 2022-06-07 }
\item \textbf{Title}: FDA panel recommends Novavax COVID vaccine be the fourth allowed for use in US
\item \textbf{Top sentence\!(weight: 0.053)}: The Novavax\!vaccine is a protein-based vaccine and includes an adjuvant to boost its effectiveness.\!
\vspace{0.05cm}
\item \underline{ 2022-06-08 }
\item \textbf{Title}: White House shifts \$10 billion in coronavirus aid to buy vaccines and treatments - The Washington Post
\item \textbf{Top sentence (weight: 0.085)}: And Republicans demanded that Democrats find ways to pay for any new pandemic spending in full rather than borrowing the money, a requirement they did not make of the billions of dollars in emergency aid for Ukraine that lawmakers approved in bipartisan fashion.
\vspace{0.05cm}
\item \underline{ 2022-06-09 }
\item \textbf{Title}: Japan's Shionogi says continuing Vietnam COVID projects after partner scandals - Reuters.com
\item \textbf{Top sentence (weight: 0.22)}: The country has administered 222.25 million doses of vaccines for its population of 98 million, according to government data.
\vspace{0.05cm}
\item \underline{ 2022-06-10 }
\item \textbf{Title}: Public school parents had a harder time with home learning during COVID
\item \textbf{Top sentence (weight: 0.062)}: That number does not include the millions more who attended virtual public-school classes from home.
\vspace{0.05cm}
\item \underline{ 2022-06-11 }
\item \textbf{Title}: This Covid wave might be the start of our `new normal,' experts say—here's what you need to know
\item \textbf{Top sentence (weight: 0.098)}: Those regional waves are often driven by different omicron subvariants — sometimes multiple at once — making the virus additionally difficult to tamp down.
\vspace{0.05cm}
\item \underline{ 2022-06-12 }
\item \textbf{Title}: COVID-19 infection rates flat
\item \textbf{Top sentence (weight: 0.17)}: The effective reproductive rate of the virus sits at about one in every state and territory, meaning one infected person is infecting at least one other person.
\vspace{0.05cm}
\item \underline{ 2022-06-13 }
\item \textbf{Title}: FDA skipped baby formula plant inspections due to COVID-19
\item \textbf{Top sentence (weight: 0.061)}: Only three of the nation's 23 facilities that make, package or distribute formula made the cut.
\vspace{0.05cm}
\item \underline{ 2022-06-14 }
\item \textbf{Title}: Drugs bounce back in Europe after COVID lockdown lull
\item \textbf{Top sentence (weight: 0.154)}: Drugs bounce back in Europe after COVID lockdown lull
\vspace{0.05cm}
\end{itemize}
}
\end{minipage}}

==> Figures/MonkeypoxOutbreak.tex <==
\fbox{\begin{minipage}{\textwidth}
{\footnotesize
\begin{itemize}[label={},leftmargin=0pt, noitemsep]
\item \underline{ 2022-06-01 }
\item \textbf{Title}: CDC Issues “Alert Level 2” For Monkeypox
\item \textbf{Top sentence (weight: 0.179)}: U.S. Rulers Orders \$119 Million Worth of Monkeypox Vaccine
\vspace{0.05cm}
\item \underline{ 2022-06-02 }
\item \textbf{Title}: Monkeypox Cases Rise to Over 550, Infections Spreading Undetected: WHO - India.com
\item \textbf{Top sentence (weight: 0.161)}: Monkeypox has not previously been described as a sexually transmitted infection, but it can be passed on by direct contact during sex.
\vspace{0.05cm}
\item \underline{ 2022-06-03 }
\item \textbf{Title}: Monkeypox in Illinois: 2nd probable case identified, is close contact of Chicago man who was IL's 1st case
\item \textbf{Top sentence (weight: 0.177)}: "Unlike COVID-19, which is a new virus, monkeypox has been around since the 1950s and the majority of cases come from central and west Africa.''
\vspace{0.05cm}
\item \underline{ 2022-06-04 }
\item \textbf{Title}: First ‘Probable’ Monkeypox Case Detected in San Francisco: Officials
\item \textbf{Top sentence (weight: 0.335)}: Monkeypox is a rare but potentially serious viral illness, usually found in west and central Africa.\!
\vspace{0.05cm}
\item \underline{ 2022-06-05 }
\item \textbf{Title}: Hundreds of monkeypox cases reported worldwide: WHO
\item \textbf{Top sentence (weight: 0.219)}: Monkeypox, which belongs to the same genus of virus as smallpox, is endemic to several countries in west and central Africa.
\vspace{0.05cm}
\item \underline{ 2022-06-06 }
\item \textbf{Title}: Monkeypox: WHO reports 780 cases
\item \textbf{Top sentence (weight: 0.146)}: Monkeypox endemic countries are Cameroon, the Central African Republic, the Democratic Republic of the Congo, Gabon, Ghana (identified in animals only), Cote d'Ivoire, Liberia, Nigeria, the Republic of the Congo, and Sierra Leone.
\vspace{0.05cm}
\item \underline{ 2022-06-07 }
\item \textbf{Title}: US cases of monkeypox reach 31
\item \textbf{Top sentence (weight: 0.16)}:Traditionally, monkeypox virus is spread by touching or getting bitten by infected wild animals in western and central Africa.
\vspace{0.05cm}
\item \underline{ 2022-06-08 }
\item \textbf{Title}: Monkeypox patient hits out at `farcical' contract tracers after being struck by virus
\item \textbf{Top sentence (weight: 0.279)}: More than 300 Brits have so far been infected with monkeypox in what is the largest outbreak in any country outside of Africa.
\vspace{0.05cm}
\item \underline{ 2022-06-09 }
\item \textbf{Title}: WHO Chief Warns Of Monkeypox Risk In Non-Endemic Countries
\item \textbf{Top sentence (weight: 0.261)}: According to WHO, Monkeypox is usually a self-limited disease and typically lasts 2 to 4 weeks.\!
\vspace{0.05cm}
\item \underline{ 2022-06-10 }
\item \textbf{Title}: UK monkeypox cases soar as infected must stay 1m from others in new `social distancing'
\item \textbf{Top sentence (weight: 0.18)}: Monkeypox has been linked to 66 deaths in Central and West Africa, where it is classified as endemic, since the start of the year.
\vspace{0.05cm}
\item \underline{ 2022-06-11 }
\item \textbf{Title}: Toronto bathhouse workers among first to be offered monkeypox vaccine - CP24 Toronto's Breaking News
\item \textbf{Top sentence (weight: 0.183)}: Monkeypox is a virus that spreads through contact with body fluids, including monkeypox lesions, contaminated clothing or bedding, or through respiratory droplets following prolonged face-to-face contact.
\vspace{0.05cm}
\item \underline{ 2022-06-12 }
\item \textbf{Title}: Canadian heading World Health Organization's fight against monkeypox - northeastNOW
\item \textbf{Top sentence (weight: 0.172)}: Has monkeypox been seen in the west before?
\vspace{0.05cm}
\item \underline{ 2022-06-13 }
\item \textbf{Title}: Combatting monkeypox on the front lines keeps fear and stigma from gay communities, advocates say
\item \textbf{Top sentence (weight: 0.242)}: Monkeypox is spread through contact with bodily fluids, including fluids from monkeypox lesions, contaminated clothing or bedding and respiratory droplets from “prolonged face-to-face contact,” according to the public health statement.
\vspace{0.05cm}
\item \underline{ 2022-06-14 }
\item \textbf{Title}: Quebec now has 132 monkeypox cases, with majority in Montreal - Global News
\item \textbf{Top sentence (weight: 0.189)}: Quebec recorded the first cases of the monkeypox in the country last month, with the first suspected infections reported on May 12 in Montreal.
\vspace{0.05cm}
\end{itemize}
}
\end{minipage}}

==> Figures/OverallAccuracy_PR.tex <==
\small
%\setlength{\tabcolsep}{11pt}
\begin{tabular}{l|cc|cc|cc}
\toprule
                                                          & \multicolumn{2}{c|}{News14} & \multicolumn{2}{c|}{WCEP18} & \multicolumn{2}{c}{WCEP19} \\
                                                          & $B^{3}$-P      & $B^{3}$-R      & $B^{3}$-P    & $B^{3}$-R    & $B^{3}$-P    & $B^{3}$-R   \\ \hline
ConStream\,\citep{constream}                                                 & 0.213          & \textbf{0.937}          & 0.341        & 0.581        & 0.349        & 0.542       \\
NewsLens\,\citep{newslens}                           & 0.357          & 0.838          & 0.422        & 0.738        & 0.469        & 0.711       \\
BatClus\,\citep{miranda}                            & 0.727          & 0.722          & 0.643        & 0.769        & 0.647        & 0.769       \\
DenSps\,\citep{staykovski}                         & 0.618          & 0.770          & 0.729        & 0.672        & 0.737        & 0.672       \\ \hline

ConStream+ST5                                             & 0.271          & 0.890          & 0.887        & 0.593        & 0.902        & 0.587       \\
NewsLens+ST5                                              & 0.571          & 0.724          & 0.666        & 0.605        & 0.690        & 0.617       \\
BatClus+ST5                                               & 0.784          & 0.712          & 0.729        & 0.699        & 0.749        & 0.692       \\
DenSps+ST5                                            & 0.601          & 0.831          & 0.674        & 0.818        & 0.613        & \textbf{0.846}       \\
\rowcolor{lightgray}
\algname{}+ST5 &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.823 \\ {\scriptsize (0.0025)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.855 \\ {\scriptsize (0.0036)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.827 \\ {\scriptsize (0.0052)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.770
\\ {\scriptsize (0.0040)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.778 
\\ {\scriptsize (0.0096)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.674 \\ {\scriptsize (0.0170)}\end{tabular}             \\ \hline

ConStream+SBERT                                              & 0.334          & 0.794          & \textbf{0.910}        & 0.575        & \textbf{0.924}        & 0.576       \\
NewsLens+SBERT                                               & 0.656          & 0.898          & 0.723        & 0.823        & 0.753        & 0.824       \\
BatClus+SBERT                                                & 0.788          & 0.770          & 0.726        & 0.796        & 0.730        & 0.804       \\
DenSps+SBERT                                             & 0.658          & 0.899          & 0.696        & 0.833        & 0.711        & 0.829       \\ 
\rowcolor{lightgray}
\algname{}+SBERT &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.887}\\ {\scriptsize (0.0012)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.871\\ {\scriptsize (0.0032)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.828\\ {\scriptsize (0.0026)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.851}
\\ {\scriptsize (0.0035)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.848
\\ {\scriptsize (0.0061)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.843
\\ {\scriptsize (0.0061)}\end{tabular}
\\ \bottomrule
\end{tabular}

==> Figures/OverallAccuracy_PR_bak.tex <==
\small
%\setlength{\tabcolsep}{11pt}
\begin{tabular}{l|cc|cc|cc}
\toprule
                                                          & \multicolumn{2}{c|}{News14} & \multicolumn{2}{c|}{WCEP18} & \multicolumn{2}{c}{WCEP19} \\
                                                          & $B^{3}$-P      & $B^{3}$-R      & $B^{3}$-P    & $B^{3}$-R    & $B^{3}$-P    & $B^{3}$-R   \\ \hline
ConStream\,\citep{constream}                                                 & 0.213          & \textbf{0.937}          & 0.341        & 0.581        & 0.349        & 0.542       \\
ConStream+ST5                                             & 0.271          & 0.890          & 0.887        & 0.593        & 0.902        & 0.587       \\
ConStream+SB                                              & 0.334          & 0.794          & \textbf{0.910}        & 0.575        & \textbf{0.924}        & 0.576       \\
NewsLens\,\citep{newslens}                           & 0.357          & 0.838          & 0.422        & 0.738        & 0.469        & 0.711       \\
NewsLens+ST5                                              & 0.571          & 0.724          & 0.666        & 0.605        & 0.690        & 0.617       \\
NewsLens+SB                                               & 0.656          & 0.898          & 0.723        & 0.823        & 0.753        & 0.824       \\
BatClus\,\citep{miranda}                            & 0.727          & 0.722          & 0.643        & 0.769        & 0.647        & 0.769       \\
BatClus+ST5                                               & 0.784          & 0.712          & 0.729        & 0.699        & 0.749        & 0.692       \\
BatClus+SB                                                & 0.788          & 0.770          & 0.726        & 0.796        & 0.730        & 0.804       \\
DenSps\,\citep{staykovski}                         & 0.618          & 0.770          & 0.729        & 0.672        & 0.737        & 0.672       \\
DenSps+ST5                                            & 0.601          & 0.831          & 0.674        & 0.818        & 0.613        & \textbf{0.846}       \\
DenSps+SB                                             & 0.658          & 0.899          & 0.696        & 0.833        & 0.711        & 0.829       \\ \hline
\rowcolor{lightgray}
\algname{}+ST5 &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.823 \\ {\scriptsize (0.0025)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.855 \\ {\scriptsize (0.0036)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.827 \\ {\scriptsize (0.0052)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.770
\\ {\scriptsize (0.0040)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.778 
\\ {\scriptsize (0.0096)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.674 \\ {\scriptsize (0.0170)}\end{tabular}             \\
\rowcolor{lightgray}
\algname{}+SB &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.887}\\ {\scriptsize (0.0012)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.871\\ {\scriptsize (0.0032)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.828\\ {\scriptsize (0.0026)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.851}
\\ {\scriptsize (0.0035)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.848
\\ {\scriptsize (0.0061)}\end{tabular} &
\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}0.843
\\ {\scriptsize (0.0061)}\end{tabular}
\\ \bottomrule
\end{tabular}

==> Figures/OverallAccuracy_bak.tex <==
\small
\centering
\setlength{\tabcolsep}{4.8pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
              & \multicolumn{3}{c}{News14} & \multicolumn{3}{c}{WCEP18} & \multicolumn{3}{c}{WCEP19} \\
              & $B^{3}$-F1   & AMI    & ARI    & $B^{3}$-F1 & AMI   & ARI   & $B^{3}$-F1 & AMI   & ARI   \\ \hline
ConStream{\scriptsize \,\citep{constream}}     & 0.314        & 0.128  & 0.069  & 0.408      & 0.444 & 0.222 & 0.400      & 0.497 & 0.292 \\
ConStream+ST5 & 0.388        & 0.282  & 0.139  & 0.707      & 0.788 & 0.660 & 0.705      & 0.793 & 0.669 \\
ConStream+SBERT  & 0.434        & 0.413  & 0.276  & 0.701      & 0.784 & 0.657 & 0.704      & 0.795 & 0.667 \\
NewsLens{\scriptsize \,\citep{newslens}}      & 0.481        & 0.309  & 0.077  & 0.527      & 0.490 & 0.117 & 0.554      & 0.529 & 0.141 \\
NewsLens+ST5  & 0.622        & 0.539  & 0.261  & 0.630      & 0.688 & 0.332 & 0.649      & 0.711 & 0.370 \\
NewsLens+SBERT   & 0.749        & 0.718  & 0.564  & 0.767      & 0.823 & 0.631 & 0.784      & 0.837 & 0.664 \\
BatClus{\scriptsize \,\citep{miranda}}       & 0.706        & 0.726  & 0.572  & 0.694      & 0.786 & 0.571 & 0.698      & 0.791 & 0.574 \\
BatClus+ST5   & 0.732        & 0.753  & 0.617  & 0.710      & 0.798 & 0.629 & 0.717      & 0.805 & 0.644 \\ 
BatClus+SBERT    & 0.764        & 0.785  & 0.648  & 0.751      & 0.835 & 0.656 & 0.759      & 0.837 & 0.657 \\ 
DenSps{\scriptsize \,\citep{staykovski}}        & 0.669        & 0.602  & 0.358  & 0.697      & 0.759 & 0.487 & 0.701      & 0.765 & 0.487 \\
DenSps+ST5    & 0.684        & 0.631  & 0.415  & 0.735      & 0.798 & 0.582 & 0.704      & 0.782 & 0.537 \\
DenSps+SBERT     & 0.750        & 0.720  & 0.567  & 0.754      & 0.824 & 0.642 & 0.762      & 0.830 & 0.660 \\ \hline 
\rowcolor{lightgray}
\algname{}+ST5
&  \renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.830 \\ {\scriptsize (0.0014)}\end{tabular}
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.847 \\ {\scriptsize (0.0016)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.756 \\ {\scriptsize (0.0034)}\end{tabular}}        
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.794 \\ {\scriptsize (0.0014)}\end{tabular}}            
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.851\\ {\scriptsize (0.0012)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.720 \\ {\scriptsize (0.0021)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.718 \\ {\scriptsize (0.0054)}\end{tabular}}            
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.803 \\ {\scriptsize (0.0026)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}} 0.633 \\ {\scriptsize (0.0045)}\end{tabular}}
\\
\rowcolor{lightgray}
\algname{}+SBERT    
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.872}\\ {\scriptsize (0.0014)}\end{tabular}}
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.879}\\ {\scriptsize (0.0014)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.809}\\ {\scriptsize (0.0028)}\end{tabular}}        
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.837}\\ {\scriptsize (0.0006)}\end{tabular}}            
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.884}\\ {\scriptsize (0.0000)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.757}\\ {\scriptsize (0.0017)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.844}\\ {\scriptsize (0.0015)}\end{tabular}}            
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.892}\\ {\scriptsize (0.0009)}\end{tabular}}       
&  {\renewcommand{\arraystretch}{0.8} \begin{tabular}[c]{@{}c@{}}\textbf{0.781}\\ {\scriptsize (0.0044)}\end{tabular}}
\\ \bottomrule


\end{tabular}


==> Figures/RussiaUkraineWar.tex <==
\fbox{\begin{minipage}{\textwidth}
{\footnotesize
\begin{itemize}[label={},leftmargin=0pt, noitemsep]
\item \underline{ 2022-06-01 }
\item \textbf{Title}: Russia-Ukraine war: List of key events, day 98
\item \textbf{Top sentence (weight: 0.075)}: The United States will send Ukraine the M142 High Mobility Artillery Rocket System (HIMARS), equipped with munitions that will allow Ukraine to launch rockets about 80km, but Ukraine will not use the missiles to hit targets on Russian territory, a senior Biden administration official said.
\vspace{0.05cm}
\item \underline{ 2022-06-02 }
\item \textbf{Title}: Russia warns West of weapons repercussions, pounds Ukraine - The Associated Press
\item \textbf{Top sentence (weight: 0.045)}: Britain on Thursday pledged to send sophisticated medium-range rocket systems to Ukraine, joining the U.S and Germany in equipping the country with some of the advanced weapons Kyiv had been begging for to shoot down aircraft and destroy artillery and supply lines.
\vspace{0.05cm}
\item \underline{ 2022-06-03 }
\item \textbf{Title}: Russia-Ukraine war: What happened today (June 3)
\item \textbf{Top sentence (weight: 0.056)}: In recent weeks, Russia has focused its efforts in the east and south, now controlling one-fifth of Ukraine.
\vspace{0.05cm}
\item \underline{ 2022-06-04 }
\item \textbf{Title}: Ukraine fighting back Sievierodonetsk, according to Luhansk governor
\item \textbf{Top sentence (weight: 0.087)}: Ukraine said it had also shot down four other cruise missiles launched from a submarine in the Black Sea – while Russia’s defence ministry said its forces shot down a Ukrainian military transport plane near Odesa.
\vspace{0.05cm}
\item \underline{ 2022-06-05 }
\item \textbf{Title}: Russia-Ukraine crisis fuelling surge in food prices – Buhari
\item \textbf{Top sentence (weight: 0.167)}: The President, Major General Muhammadu Buhari (retd.), on Saturday in Accra said ongoing invasion of Ukraine by Russia had led to a surge in the prices of many commodities, including foodstuffs.
\vspace{0.05cm}
\item \underline{ 2022-06-06 }
\item \textbf{Title}: Russia-Ukraine war: List of key events, day 103
\item \textbf{Top sentence (weight: 0.081)}: The UK said it will supply Ukraine with M270 multiple-launch rocket systems that can attack targets up to 80km (50 miles) away in a move coordinated with the United States.
\vspace{0.05cm}
\item \underline{ 2022-06-07 }
\item \textbf{Title}: Russia's UN envoy walks out after Moscow blamed for food crisis
\item \textbf{Top sentence (weight: 0.092)}: Kyslytsya said the question has become more relevant since four Russian missiles hit a plant in the capital Kyiv on Sunday, where freight cars that carry grain to Ukrainian ports were being repaired.
\vspace{0.05cm}
\item \underline{ 2022-06-08 }
\item \textbf{Title}: No progress at Russia-Turkey talks on Ukraine grain exports
\item \textbf{Top sentence (weight: 0.08)}: But Russia's chief diplomat blamed Ukraine for the situation.
\vspace{0.05cm}
\item \underline{ 2022-06-09 }
\item \textbf{Title}: Is Russia inching towards victory in Ukraine’s Donbas region?
\item \textbf{Top sentence (weight: 0.036)}: NATO countries have worked together to keep Ukraine armed but are still reluctant to give Ukraine weapons systems that can attack targets inside Russia, fearing escalation involving a probable Russian declaration of war that would lead to the total focus of its economy on the conflict.
\vspace{0.05cm}
\item \underline{ 2022-06-10 }
\item \textbf{Title}: Putin's bodyguards collect his poop on trips abroad and take it back to Russia with them, report says
\item \textbf{Top sentence (weight: 0.159)}: Amid Russia's invasion of Ukraine, speculation has grown that Putin, who has recently missed a number of routine events, is unwell, and several reports have claimed that he is being treated for a variety of serious conditions.
\vspace{0.05cm}
\item \underline{ 2022-06-11 }
\item \textbf{Title}: Putin Draws Parallels Between War In Ukraine And 18th Century Conquests Of Peter The Great
\item \textbf{Top sentence (weight: 0.106)}: Putin has sought to justify Russia's invasion of Ukraine by asserting that Ukraine has no real national identity or tradition of statehood, while Moscow says it acted to disarm and "denazify'' Ukraine.
\vspace{0.05cm}
\item \underline{ 2022-06-12 }
\item \textbf{Title}: Matteo Salvini defends himself over plans for Russian-funded Moscow trip
\item \textbf{Top sentence (weight: 0.166)}: “I met the Ukrainian ambassador to show solidarity, and the Russian one to ask for a ceasefire.''
\vspace{0.05cm}
\item \underline{ 2022-06-13 }
\item \textbf{Title}: Putin Nemesis Warns of Sinister Twist in Russian Attack Plan
\item \textbf{Top sentence (weight: 0.06)}: Russian President Vladimir Putin has been waging a devastating war in Ukraine for over three months now.`
\vspace{0.05cm}
\item \underline{ 2022-06-14 }
\item \textbf{Title}: Pope blasts Russian `cruelty,' lauds Ukrainian `heroism'
\item \textbf{Top sentence (weight: 0.148)}: Pope blasts Russian `cruelty,' lauds Ukrainian `heroism'
\vspace{0.05cm}
\end{itemize}
}
\end{minipage}}
